A piece-wise constant approximation for non-conjugate Gaussian Process models

Gaussian Processes (GPs) are a versatile and popular method in Bayesian Machine Learning. A common modification are Sparse Variational Gaussian Processes (SVGPs) which are well suited to deal with large datasets. While GPs allow to elegantly deal with Gaussian-distributed target variables in closed form, their applicability can be extended to non-Gaussian data as well. These extensions are usually impossible to treat in closed form and hence require approximate solutions. This paper proposes to approximate the inverse-link function, which is necessary when working with non-Gaussian likelihoods, by a piece-wise constant function. It will be shown that this yields a closed form solution for the corresponding SVGP lower bound. In addition, it is demonstrated how the piece-wise constant function itself can be optimized, resulting in an inverse-link function that can be learnt from the data at hand.

==> sections/033_deepgp.tex <==
Introduced in \cite{damianou2013deep}, Deep Gaussian Processes (DGP) apply the idea of 'deep', stacked models to the GP domain. For a DGP with $2$ layers, we are interested in the posterior distribution

\begin{equation}\label{dgpposterior}
    p(f_1,f_2|X,y)\propto p(y|f_2)p(f_2|f_1)p(f_1|X).
\end{equation}

with

\begin{gather}
    p(f_1|X) = \mathcal{GP}(f_1|0,k_1(x,x')))\\
    p(f_2|f_1) = \mathcal{GP}(f_2|0,k_2(f_1,f_1')). \label{dgpsecond}
\end{gather}

The propagation of $f_1$ through $k_2$ in \eqref{dgpsecond} results in an intractable posterior distribution in \eqref{dgpposterior}. We can again work with inducing variables to approximate the true posterior via variational inference:

\begin{gather}
    q(f_1,f_{m,1})= p(f_1|f_{m,1})q(f_{m,1}) \\
    q(f_2,f_{m,2})= \int p(f_2|f_{m,2},f_1,f_{m,1})q(f_{m,2})q(f_1,f_{m,1}) df_1 df_{m,1}
\end{gather}

Using the approach in \cite{salimbeni2017doubly}, we obtain the following lower bound:

\begin{equation}\label{elbodgp}
    \begin{gathered}
        ELBO = \sum_{i=1}^n\mathbb{E}_{p(f|f_M)q(f_M)}\left[\log p(y_{(i)}|g(f_{(i)}))\right]-KL(q(f_M)||p(f_M)) \\
        \approx \sum_{i=1}^n\sum_{k=1}^{K}\log  p(y_{(i)}|a_k) P(l_k < f_{(i)}|f_M < u_k) -KL(q(f_M)||p(f_M))
        
    \end{gathered}
\end{equation}


\cite{salimbeni2017doubly}, \textbf{Remark 2}:

\begin{equation}\label{elbodgpapprox}
    \begin{gathered}
        ELBO = \sum_{i=1}^n\mathbb{E}_{p(f|f_M)q(f_M)}\left[\log p(y_{(i)}|g(f_{(i)}))\right]-KL(q(f_M)||p(f_M)) \\
        \approx \sum_{i=1}^n\sum_{k=1}^{K}\log  p(y_{(i)}|a_k) P(l_k < f_{(i)}|f_M < u_k) -KL(q(f_M)||p(f_M))
        
    \end{gathered}
\end{equation}
